OmniCompass: A Holistic Benchmark for Omni-Modal Video Grounding and Understanding

With the rapid development of multimodal large language models (MLLMs), evaluating their video understanding capabilities has become increasingly important. Existing video understanding benchmarks cover only part of the evaluation dimensions, limiting systematic diagnosis of omni-modal video understanding. We introduce OmniCompass, a holistic benchmark for omni-modal video grounding and understanding. OmniCompass defines two evaluation tracks: OmniCompass-VL assesses vision-language models on tasks requiring visual evidence, while OmniCompass-AV assesses omni-modal models on tasks requiring joint audio-visual evidence. Each track includes three complementary tasks: temporal grounding (TG), spatial grounding (SG), and question answering (QA), assessing when a referenced target appears, where it is, and what happens. QA covers five perception and three reasoning categories in OmniCompass-VL, and three perception and two reasoning categories in OmniCompass-AV. OmniCompass-VL contains 820 videos and 2,460 instances across domains and three duration types: short, medium, and long. A narrative- and audio-rich subset forms OmniCompass-AV with 240 videos and 720 instances. Each instance is evaluated under two paired settings: text-only and text+image, specifying the same target through text and visual-language guidance. All instances are manually annotated with multi-round quality verification. Evaluations of 50 MLLMs show that open-source models still lag behind proprietary counterparts, particularly in audio-visual understanding. Precise temporal and spatial grounding remains challenging even for leading models, and their predictions still exhibit inconsistencies across the paired target specifications.

==> Sections/6_Statements.tex <==
\subsection*{AI Use Statement}
As described in Section~\ref{sec:benchmark} and Appendix~\ref{sec:appendix_benchmark_construction}, we use \texttt{Qwen3-VL-8B-Instruct} to generate detailed video captions and structured descriptions for candidate screening.
LLM-based tools also assist with manuscript polishing and figure preparation based on our existing data.
The authors review the AI-assisted content and take responsibility for the accuracy and integrity of the paper.

\subsection*{Reproducibility Statement}
Benchmark construction, annotation protocols, and evaluation metrics are described in Section~\ref{sec:benchmark}.
Experimental setup is provided in Section~\ref{sec:Experiments}.
Details of data filtering and quality verification, along with evaluation prompts and output formats for both tracks, are provided in Appendix~\ref{sec:appendix_benchmark_construction}.

==> Tables/prompts/qwen_scoring.tex <==
\begin{table*}[t]
\caption{
\textbf{Mapping from structured video profiling outputs to task-oriented scoring signals.}
We summarize how the structured video profiling outputs produced by \texttt{Qwen3-VL-8B-Instruct} are converted into intermediate statistics and then used to compute the four score components.
}
\label{tab:qwen_scoring}
\centering
\setlength{\tabcolsep}{4.2pt}
\renewcommand{\arraystretch}{1.08}
\resizebox{\textwidth}{!}{
\begin{threeparttable}
\begin{tabular}{p{2.5cm} p{3.8cm} p{6.1cm} p{4.8cm}}
\toprule
\textbf{Component} & \textbf{Derived profiling fields} & \textbf{Computation} & \textbf{Intuition} \\
\midrule

\textbf{Reference Necessity ($R$)}
& \texttt{entity\_count}, \texttt{action\_count}, \texttt{attribute\_count}, \texttt{scene\_count}, repeated actions
& We first compute \textit{ambiguity} and \textit{richness}. Ambiguity increases with multiple candidate entities, repeated actions, scene variation, and potential attribute confusion. Richness increases with broader coverage over entity, action, attribute, and scene signals. We then combine them as
$
R = 10 \cdot \left(0.60A + 0.20B + 0.20AB\right),
$
where $A$ and $B$ are the normalized ambiguity and richness scores.
& Measures whether external referential cues are needed to uniquely specify the target. \\

\textbf{Grounding Suitability ($G$)}
& \texttt{entity\_count}, \texttt{action\_count}, \texttt{attribute\_count}, \texttt{scene\_count}
& We estimate temporal grounding potential from action and scene counts, spatial grounding potential from entity and attribute counts, and question answering potential from action and scene-related complexity. The final score is
$
G = 10 \cdot \mathrm{avg}(P_{\text{TG}}, P_{\text{SG}}, P_{\text{QA}}).
$
& Measures whether the video can support constructing TG, SG, and VideoQA instances. \\

\textbf{Temporal-Spatial Utility ($T$)}
& video duration, \texttt{entity\_count}, \texttt{action\_count}, \texttt{scene\_count}
& We combine a duration term and a variation term:
$
T = 10 \cdot \left(0.60D + 0.40V\right),
$
where $D$ is a log-normalized duration score and $V$ is the average of normalized action, scene, and entity variation.
& Measures whether the video provides sufficient temporal span and visual variation for evidence localization. \\

\textbf{Evidence Diversity ($E$)}
& \texttt{entity\_count}, \texttt{action\_count}, \texttt{attribute\_count}, \texttt{scene\_count}
& We compute normalized entropy over the four evidence counts:
$
E = 10 \cdot H_{\text{norm}}(c_{\text{ent}}, c_{\text{act}}, c_{\text{att}}, c_{\text{scn}}).
$
& Measures whether referential evidence is distributed across multiple cue types rather than concentrated in a single source. \\

\midrule
\textbf{Final Score ($S$)}
& $R, G, T, E$
& $
S = 0.35R + 0.25G + 0.25T + 0.15E
$
& Encourages videos that require diverse referential cues, support TG/SG/VideoQA construction, and provide diverse evidence for annotation. \\

\bottomrule
\end{tabular}
\vspace{-4mm}
\end{threeparttable}
}
\end{table*}


==> Tables/prompts/qwen_structured_prompt.tex <==
\begin{figure*}[h]
\centering
\begin{omniprompt}{Structured Video Profiling Prompt}
\small
You are a factual video captioning and structured extraction assistant.\\
Only describe what is clearly visible or audible. Do NOT guess.\\
Output ONE valid JSON object only.\\
Do NOT place JSON inside any field.
\smallskip
\textbf{Write:}
\begin{enumerate}[leftmargin=18pt, topsep=2pt, itemsep=0pt, parsep=0pt]
\item \texttt{detailed\_description}: 3--6 sentences, time order.
\item \texttt{entity}: list categories with \texttt{instance\_count} and short notes.
\item \texttt{action}: up to 12 distinct temporally localizable action variants.
\item \texttt{attribute}: up to 12 distinct visible cues.
\item \texttt{scene}: up to 6 distinct phases, shots, or contexts.
\item \texttt{counts}: \texttt{entity} = sum of \texttt{entity.instance\_count}; others = list lengths.
\end{enumerate}
{\normalfont\bfseries Required JSON Output\par}
\smallskip
\footnotesize\ttfamily
Return JSON with EXACT keys:\\
\{\\
"detailed\_description":"...",\\
"entity":[\{"category":"...","instance\_count":0,"notes":"..."\}],\\
"action":["..."],\\
"attribute":["..."],\\
"scene":["..."],\\
"counts":\{"entity":0,"action":0,"attribute":0,"scene":0\}\\
\}
\end{omniprompt}
\caption{\textbf{Structured video profiling prompt used with \texttt{Qwen3-VL-8B-Instruct}.}}
\label{fig:qwen_structured_prompt}
\end{figure*}

==> Tables/results_av_old.tex <==
\begin{table*}[t]
\caption{
\textbf{Results on the OmniCompass-AV track.}
We evaluate proprietary and open-source omni-modal MLLMs on TG, SG, and QA using native video with synchronized audio;
\textbf{Frames} gives the retained frame count.
Entries report \textit{Text}/\textit{Text+Image} for the two target specifications.
Overall averages TG $m_{\mathrm{tIoU}}$, SG $m_{\mathrm{sIoU}}$, and QA
accuracy within each setting.
}
\vspace{-2mm}
\label{tab:results_av}
\centering
\setlength{\tabcolsep}{4pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lc|cccc|cccc|c|c}
\toprule
\multirow{2}{*}{\textbf{Models}} &
\multirow{2}{*}{\textbf{Frames}} &
\multicolumn{4}{c|}{\textbf{Temporal Grounding (TG)}} &
\multicolumn{4}{c|}{\textbf{Spatial Grounding (SG)}} &
\textbf{QA} &
\multirow{2}{*}{\textbf{Overall}} \\
\cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-11}
& & \textbf{Acc.@0.3} & \textbf{Acc.@0.5} & \textbf{Acc.@0.7} & \textbf{$m_{\mathrm{tIoU}}$}
& \textbf{Acc.@0.3} & \textbf{Acc.@0.5} & \textbf{Acc.@0.7} & \textbf{$m_{\mathrm{sIoU}}$}
& \textbf{Accuracy}
& \\
\midrule
\rowcolor{omniyellow}
\multicolumn{12}{l}{\textbf{\textit{Proprietary Omni-modal MLLMs}}} \\
\midrule

Gemini-3.8-Flash & 64 & 70.3/67.8 & 46.9/48.1& 25.9/27.2& 46.4/45.9 & 77.0/74.5 & 63.2/62.8 & 48.5/48.1 & 59.8/58.7 & -- & -- \\

% native 64 frames
% Gemini-3.8-Flash & 64 & 56.9/58.6 & 39.3/41.4 & 20.9/20.1 & 38.2/39.1 & 36.4/35.6 & 13.0/12.1 & 4.2/4.2 & 24.0/24.4 & -- & -- \\

Gemini-3.1-Pro & 64 & 24.7/25.5 & 15.1/17.6& 8.8/8.4 & 16.6/17.7 & 74.1/76.6 & 54.8/56.1 & 33.1/31.8 & 52.0/52.1 & -- & -- \\

Doubao-Seed-2.0-lite-260428 & 64 & 22.1/17.1 & 13.3/8.3 & 5.8/3.3 & 16.9/13.2 & 72.9/75.0 & 56.3/52.9 & 35.4/33.3 & 53.3/51.8 & -- & -- \\

Doubao-Seed-2.0-mini-260428 & 64 & 9.6/4.6  & 4.2/3.3  & 1.7/0.4 & 6.4/3.8 & 44.6/45.4 & 27.1/25.4 & 10.0/7.1  & 28.6/28.8 & -- & -- \\

Qwen3.8-Omni-Flash & 64 & 41.9/43.6 & 26.4/28.4 & 11.9/13.8 & 29.3/30.8 & 78.1/76.4 & 60.1/59.1 & 42.5/41.3 & 56.8/55.8 & -- & -- \\

Qwen3.5-Omni-Plus & 64 & 30.7/31.1 & 18.0/14.9 & 7.5/7.0 & 21.0/21.1 & 76.3/74.9 & 61.8/60.8 & 39.9/41.9 & 55.5/55.6 & -- & -- \\

% native 64 frames
% Qwen3.5-Omni-Plus & 64 & 29.0/31.9 & 16.0/18.9 & 6.3/4.6 & 19.3/20.1 & 41.2/44.7 & 14.7/24.9 & 3.8/6.3 & 26.3/29.3 & -- & -- \\

Qwen3.5-Omni-Flash & 64 & 16.3/14.2 & 6.7/7.9 & 2.1/3.8 & 10.6/10.1 & 64.2/67.2 & 49.2/51.3 & 31.7/34.0 & 44.2/47.0 & -- & -- \\


\midrule
\rowcolor{omnigreen}
\multicolumn{12}{l}{\textbf{\textit{Open-Source Omni-modal MLLMs}}} \\
\midrule

MiMo-V2.5 & 64 & 12.6/11.8 & 6.3/8.6  & 3.4/3.2  & 9.4/8.7   & 56.6/57.2 & 29.2/33.2 & 6.4/10.1  & 34.9/36.0 & -- & -- \\

% native 64 frames
% MiMo-V2.5 & 64 & 38.1/36.6 & 28.9/22.3 & 12.6/7.6 & 25.2/22.9 & 22.5/36.7 & 6.3/12.9 & 0.4/1.3 & 17.6/24.0 & -- & -- \\


Qwen3-Omni-30B-A3B & 32 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

Qwen2.5-Omni-7B & 32 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

Qwen2.5-Omni-4B & 32 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

video-SALMONN 2+ 72B & 32 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

video-SALMONN 2+ 7B & 32 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

MiniCPM-o-4.5-8B & 32 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

Ola-7B & 32 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

VideoLLaMA2-7B & 32 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

VITA-1.5-7B & 16 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
\bottomrule
\end{tabular}%
}
\vspace{-4mm}
\end{table*}

==> Tables/results_vl_old.tex <==
\begin{table*}[t]
\caption{
\textbf{Results on the OmniCompass-VL track.}
We evaluate MLLMs on TG, SG, and QA without audio; \textbf{Frames} counts
uniformly sampled frames, each preceded by a timestamp.
Entries report \textit{Text}/\textit{Text+Image}; in the latter, the reference
image immediately follows all sampled video frames.
Overall averages TG $m_{\mathrm{tIoU}}$, SG $m_{\mathrm{sIoU}}$, and QA
accuracy per setting.
}
\vspace{-2mm}
\label{tab:results_vl}
\centering
\setlength{\tabcolsep}{4pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lc|cccc|cccc|c|c}
\toprule
\multirow{2}{*}{\textbf{Models}} &
\multirow{2}{*}{\textbf{Frames}} &
\multicolumn{4}{c|}{\textbf{Temporal Grounding (TG)}} &
\multicolumn{4}{c|}{\textbf{Spatial Grounding (SG)}} &
\textbf{QA} &
\multirow{2}{*}{\textbf{Overall}} \\
\cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-11}
& & \textbf{Acc.@0.3} & \textbf{Acc.@0.5} & \textbf{Acc.@0.7} & \textbf{$m_{\mathrm{tIoU}}$}
& \textbf{Acc.@0.3} & \textbf{Acc.@0.5} & \textbf{Acc.@0.7} & \textbf{$m_{\mathrm{sIoU}}$}
& \textbf{Accuracy}
& \\
\midrule
\rowcolor{omniyellow}
\multicolumn{12}{l}{\textbf{\textit{Proprietary MLLMs}}} \\
\midrule

Gemini-3.8-Flash & 64 & 47.6/50.4 & 33.8/32.7 & 15.8/17.0 & 32.6/33.5 & 53.2/62.8 & 37.5/41.6 & 21.2/22.6 & 37.7/41.8 & 73.3/76.6 & 47.9/50.6 \\


Gemini-3.1-Pro & 64 & 37.2/38.7 & 24.9/24.9 & 12.7/11.8 & 25.6/26.6 & 56.2/58.3 & 34.9/35.2 & 16.5/16.6 & 36.5/37.3 & 71.4/73.6 & 44.5/45.9 \\


% Doubao-Seed-2.1-pro-260915 & 64 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

% Doubao-Seed-2.1-turbo-260628 & 64 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

Doubao-Seed-2.0-pro-260215 & 64 & 44.0/44.1 & 30.7/31.0 & 14.4/15.1 & 30.6/30.9 & 55.0/54.9 & 30.6/31.7 & 13.8/13.7 & 34.9/35.3 & 74.5/73.0 & 46.6/46.4 \\

% Grok 4.6 & 64 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

GPT-5.5 & 49 & 38.7/40.9 & 23.3/24.5 & 10.9/12.6 & 26.0/27.5 & 38.7/39.1 & 20.6/20.5 & 7.0/7.0 & 26.4/26.3 & 67.9/70.2 & 40.1/41.3 \\

GPT-5.6-Luna & 49 & 36.5/36.3 & 21.0/21.3 & 10.7/10.7 & 24.7/24.8 & 50.0/51.2 & 27.3/28.9 & 11.6/10.2 & 32.2/33.1 & 65.5/64.6 & 40.8/40.8 \\

GPT-5.6-Terra & 49 & 34.1/39.1 & 20.1/23.7 & 10.5/10.9 & 24.1/26.3 & 41.3/41.3 & 19.4/20.9 & 6.0/6.0 & 26.3/26.6 & 68.4/69.5 & 39.6/40.8 \\

GPT-5.6-Sol & 49 & 40.4/44.8 & 25.2/28.7 & 12.4/15.1 & 27.2/30.5 & 53.7/52.4 & 31.7/29.8 & 11.6/12.8 & 34.8/33.8 & 69.5/69.1 & 43.8/44.5 \\

GPT-6-Astra & 49 & 43.3/45.6 & 30.0/30.3 & 16.7/17.4 & 30.9/31.7 & 55.7/57.1 & 34.6/35.9 & 19.6/19.4 & 37.8/38.3 & 69.4/65.6 & 46.0/45.2 \\

Qwen3.8-Max & 64 & 43.9/45.8 & 29.3/30.3 & 16.1/17.0 & 30.7/32.2 & 52.2/52.6 & 30.1/32.1 & 13.0/12.6 & 33.9/34.0 & 72.4/72.5 & 45.7/46.2 \\

Qwen3.8-Flash & 64 & 42.8/45.8 & 28.5/30.1 & 14.6/15.1 & 29.5/30.6 & 44.8/46.7 & 22.6/24.4 & 7.4/7.6 & 28.8/29.3 & 69.2/71.0 & 42.5/43.6 \\


\midrule
\rowcolor{omniblue}
\multicolumn{12}{l}{\textbf{\textit{Open-Source MLLMs}}} \\
\midrule

MiMo-V2.5 & 64 & 31.7/29.4 & 17.8/18.6 & 8.5/9.9 & 21.6/20.8 & 32.7/33.2 & 14.2/15.3 & 3.5/3.4 & 21.9/22.3 & 62.0/60.8 & 35.2/34.7 \\

DeepSeek-V4.1-Flash & 64 & 28.2/28.9 & 15.7/17.4 & 8.8/9.3 & 19.1/19.4 & 27.0/26.2 & 11.5/11.6 & 2.1/2.1 & 18.1/17.9 & 66.2/64.6 & 34.5/34.0 \\

GLM-5.3-Flash & 64 & 38.0/36.7 & 24.4/23.0 & 10.9/9.9 & 25.5/24.4 & 36.0/37.8 & 15.7/14.6 & 2.9/3.3 & 22.9/23.5 & 68.3/68.7 & 38.9/38.9 \\

Kimi-K3 & 64 & 39.7/41.0 & 23.5/24.6 & 12.6/13.2 & 27.1/27.7 & 50.8/53.7 & 30.0/31.6 & 11.8/12.1 & 33.3/35.2 & 73.0/72.9 & 44.5/45.3 \\

Qwen3.5-397B-A17B & 64 & 41.9/41.2 & 28.9/28.5 & 14.1/14.9 & 28.6/28.7 & 51.9/52.4 & 28.2/29.6 & 12.5/12.4 & 33.4/33.7 & 67.7/69.6 & 43.3/44.0 \\

Qwen3.5-122B-A10B & 64 & 43.2/42.1 & 27.2/27.2 & 14.5/14.6 & 29.7/29.1 & 39.4/38.2 & 20.0/19.4 & 6.4/6.4 & 25.2/25.2 & 62.6/62.5 & 39.2/38.9 \\

% Qwen3-VL-235B-A22B-Thinking & 64 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

Qwen3-VL-235B-A22B-Instruct & 64 & 40.3/36.9 & 27.0/25.4 & 15.2/11.3 & 28.5/26.0 & 39.6/37.3 & 18.6/18.8 & 5.6/6.4 & 26.0/25.0 & 68.4/65.3 & 41.0/38.8 \\

Qwen3.8-27B & 32 & 29.9/32.1 & 17.5/19.1 & 7.9/8.3 & 20.3/22.2 & 36.6/39.7 & 16.2/19.0 & 5.5/6.0 & 23.9/25.4 & 64.8/62.6 & 36.3/36.7 \\

Qwen3.6-35B-A3B & 32 & 27.5/29.0 & 18.7/18.8 & 9.2/7.5 & 19.8/19.7 & 40.9/41.5 & 20.9/19.1 & 8.3/7.4 & 26.8/26.4 & 59.5/59.9 & 35.4/35.3 \\

Qwen3.6-27B & 32 & 30.4/29.2 & 20.5/18.8 & 9.3/9.1 & 21.5/20.4 & 31.5/32.8 & 14.4/15.8 & 5.2/6.5 & 20.7/22.2 & 62.5/61.2 & 34.9/34.6 \\

Qwen3.5-35B-A3B & 32 & 27.6/27.1 & 17.3/16.4 & 8.6/8.0 & 19.5/18.7 & 32.5/32.6 & 13.3/13.4 & 4.4/4.7 & 21.2/21.9 & 61.3/60.9 & 34.0/33.8 \\

Qwen3.5-27B & 32 & 30.8/29.1 & 19.4/18.0 & 8.8/8.2 & 22.0/21.1 & 26.1/26.6 & 11.3/11.5 & 3.2/3.7 & 18.6/19.1 & 61.5/58.4 & 34.0/32.9 \\

Qwen3.5-9B & 32 & 29.8/25.1 & 17.4/14.4 & 7.4/6.3 & 20.2/16.6 & 34.0/34.0 & 16.8/16.8 & 5.5/5.7 & 22.3/22.3 & 58.5/55.2 & 33.7/31.4 \\

Qwen3.5-4B & 32 & 28.2/21.8 & 16.6/12.4 & 7.7/6.8 & 19.5/15.3 & 28.3/25.9 & 13.0/11.6 & 4.9/3.4 & 18.9/17.1 & 55.7/54.0 & 31.4/28.8 \\

Qwen3-VL-30B-A3B-Instruct & 32 & 27.6/21.8 & 16.8/12.4 & 8.2/5.4 & 19.5/14.9 & 32.9/27.6 & 15.2/12.9 & 5.5/5.8 & 22.1/19.6 & 54.1/49.6 & 31.9/28.0 \\

Qwen3-VL-8B-Instruct & 32 & 22.8/19.9 & 13.2/11.1 & 4.8/4.0 & 16.3/13.9 & 30.0/26.5 & 13.8/12.4 & 5.0/5.0 & 20.4/19.3 & 59.9/56.7 & 32.2/29.9 \\

Qwen3-VL-4B-Instruct & 32 & 24.4/18.9 & 13.8/10.5 & 5.5/4.3 & 16.8/13.0 & 16.7/15.4 & 6.6/5.6 & 1.8/2.0 & 13.4/12.2 & 57.3/56.0 & 29.2/27.1 \\

InternVL3.5-38B & 32 & 23.7/19.4 & 13.0/10.5 & 5.0/4.6 & 16.3/13.6 & 1.1/1.5 & 0.2/0.1 & 0.0/0.0 & 2.5/2.5 & 61.3/58.4 & 26.7/24.8 \\

% 579 条 8k thinking 截断请求全部排除，不进入分母。139条 thinking 仍耗尽32K。
Keye-VL-2.0-30B-A3B & 32 & 21.7/18.4 & 12.8/11.0 & 5.8/5.6 & 15.0/13.0 & 12.0/14.1 & 2.7/3.3 & 0.1/0.6 & 11.5/12.1 & 59.6/61.5 & 28.7/28.8 \\

TimeLens2-8B & 32 & 30.2/27.1 & 20.7/18.2 & 7.4/6.8 & 20.8/18.5 & 8.9/7.7 & 2.4/2.6 & 1.0/0.9 & 9.1/8.0 & 59.5/57.0 & 29.8/27.8 \\

TimeLens-8B & 32 & 31.2/25.9 & 22.4/18.5 & 8.4/6.7 & 21.4/18.1 & 8.5/8.8 & 2.4/2.8 & 0.5/0.6 & 8.2/8.7 & 57.7/55.5 & 29.1/27.4 \\

LLaVA-OneVision-2-8B & 32 & 23.7/15.4 & 15.4/10.7 & 6.2/4.8 & 15.8/11.2 & 5.6/5.2 & 0.9/1.1 & 0.2/0.2 & 7.1/6.7 & 57.9/52.4 & 26.9/23.4 \\

LLaVA-Video-7B & 32 & 6.2/4.1 & 1.6/2.1 & 0.6/0.6 & 4.3/3.1 & 0.0/0.4 & 0.0/0.0 & 0.0/0.0 & 0.5/0.5 & 55.0/50.7 & 19.9/18.1 \\

LLaVA-OneVision-7B & 32 & 6.0/3.2 & 2.6/1.7 & 0.7/0.4 & 4.6/2.4 & 0.4/0.2 & 0.0/0.0 & 0.0/0.0 & 2.0/1.6 & 50.7/47.9 & 19.1/17.3 \\

\bottomrule
\end{tabular}%
}
% \vspace{-4mm}
\end{table*}
